EnvPoser: Environment-aware Realistic Human Motion Estimation from Sparse Observations with Uncertainty Modeling

Estimating full-body motion using the tracking signals of head and hands from VR devices holds great potential for various applications. However, the sparsity and unique distribution of observations present a significant challenge, resulting in an ill-posed problem with multiple feasible solutions (i.e., hypotheses). This amplifies uncertainty and ambiguity in full-body motion estimation, especially for the lower-body joints. Therefore, we propose a new method, EnvPoser, that employs a two-stage framework to perform full-body motion estimation using sparse tracking signals and pre-scanned environment from VR devices. EnvPoser models the multi-hypothesis nature of human motion through an uncertainty-aware estimation module in the first stage. In the second stage, we refine these multi-hypothesis estimates by integrating semantic and geometric environmental constraints, ensuring that the final motion estimation aligns realistically with both the environmental context and physical interactions. Qualitative and quantitative experiments on two public datasets demonstrate that our method achieves state-of-the-art performance, highlighting significant improvements in human motion estimation within motion-environment interaction scenarios.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/old_intro.tex <==
\section{Introduction}
\label{sec:intro}
% xspc

In recent years, motion capture algorithms using sparse tracking signals have achieved significant progress across various research fields, establishing themselves as essential technologies for applications such as motion-sensing games and immersive VR/AR experiences~\cite{huang2018deep, kaufmann2021pose, yi2022physical}.
% establishing themselves as a crucial technology for motion capture in applications like 
%\IEEEPARstart{R}{econstructing} a user's motion using only wearable devices is essential for many Virtual Reality (VR) applications, such as in motion-sensing games and immersive social interactions. 
With the rapid development of VR devices, full-body motion estimation algorithms based on head-mounted displays (HMDs) have shown great application potential. However, devices like PICO and Quest typically provide sparse tracking signals of the head and hands, presenting challenges in estimating the full-body motion from these limited observations.

% Devices like Pico and Meta Quest typically provide the positional information for the head, left hand, and right hand, presenting challenges in inferring full-body motion from this limited observational data. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{sec/figure/Intro.png} % Adjust the width as needed
    \caption{
      Our proposed EnvPoser method estimates the human motion with the sparse tracking signals and a pre-reconstruction environment, which could be reconstructed using HMD's cameras during the device initialization phase.
    }
    \label{fig:1}
    \vspace{-5mm}
    
\end{figure}

Current sparse-observation-based human motion estimation methods typically rely on large-scale motion capture datasets, such as AMASS~\cite{mahmood2019amass}, to capture full-body motion through regression~\cite{jiang2022avatarposer, zheng2023realistic} or generative models~\cite{feng2024stratified, du2023avatars}.
Alternatively, some methods~\cite{xxx} turn to physics engines and reinforcement learning to synthesize full-body motion, bypassing dataset dependency.
Despite these significant advances, full-body motion estimation from sparse tracking signals remains challenging due to the lack of comprehensive joint measurements, particularly for the lower body. This limitation frequently results in multi-hypothesis motion corresponding to the same sparse observations, making full-body motion estimation an ill-posed problem.

% Consequently, even with effective neural networks and large motion datasets, capturing the complex kinematic characteristics of human motion poses continues to pose a significant challenge. The sparsity of observational data often results in missing information for full-body joint measurements, particularly when estimating lower-body joints. This situation frequently leads to a multi-hypothesis nature in motion estimation, where multiple distinct postures can correspond to the same sensor input.
% The lack of comprehensive joint measurements, especially for the lower body, frequently results in a multi-hypothesis issue, where multiple distinct poses may correspond to the same sensor input.

To address this ambiguity, our approach implicitly models joint estimation uncertainty within the network and uses sampling to represent multiple plausible motion hypotheses. However, reducing this uncertainty remains a significant challenge for full-body motion estimation with sparse observations. Some existing studies propose adding sensors to the pelvis and legs to mitigate motion estimation uncertainty~\cite{ponton2023sparseposer, dai2024hmd, ponton2024dragposer}. While additional sensors can improve the accuracy and robustness of full-body motion estimation, this approach may negatively impact user experience due to the increased hardware requirements~\cite{huang2018deep, jiang2022transformer, yi2022physical, zhang2024dynamic}.

% While these methods enhance the accuracy and robustness of motion capture through increased sensor measurements, they are more suitable for sparse IMU-based motion reconstruction studies~\cite{huang2018deep, jiang2022transformer, yi2022physical, zhang2024dynamic}. Although this strategy can yield more accurate reconstructions, it may negatively impact user experience in everyday applications.

% Due to the sparsity of observational data, there is inevitably missing information for full-body joint measurements, particularly when estimating lower body joints. This often results in the multi-hypothesis nature of poses, where multiple distinct postures can correspond to the same sensor input. To effectively capture this ambiguity in pose estimation, we implicitly model it through uncertainty. Our approach quantifies the uncertainty in joint estimation within the network and leverages sampling to represent multiple plausible motion reconstruction hypotheses.

%Due to the sparsity of the observational data, measurement information for the full-body joints inevitably suffers from gaps, especially in estimating the lower body joints, which may lead to multiple different poses matching the same sensor input and increasing uncertainty in the pose solution space.

%或许可以在描述下不好的现状现象

% However, reducing the uncertainty in pose estimation will be a significant challenge to motion reconstruction with sparse observations. To address this issue, existing researches have proposed adding additional sensors to the pelvis and legs to reduce pose estimation uncertainty~\cite{ponton2023sparseposer, dai2024hmd, ponton2024dragposer}. These methods enhance the accuracy and robustness of motion capture by increasing sensor measurements. However, adding sensors is more suitable for sparse IMU-based motion reconstruction studies~\cite{huang2018deep, jiang2022transformer, yi2022physical, zhang2024dynamic}. Although this strategy can yield more accurate motion pose reconstructions, it may affect user experience in everyday applications.

An alternative approach to addressing the inherent ambiguity in sparse observations is to incorporate additional environmental constraints, which, unlike adding sensors, does not impact the user’s wearable experience. By leveraging prior knowledge of the environment, full-body motion estimates can be refined when observations are limited, as environmental cues can help correct body poses that may otherwise appear ambiguous.
However, effectively utilizing environmental constraints presents its own challenges, as existing methods~\cite{tang2024unified, zheng2023realistic} often simplify human-environment interactions to basic foot-to-ground contact, overlooking the complexities of everyday interactions. In reality, individuals frequently engage in more complex interactions with their surroundings. In this work, we address these challenges by incorporating human-environment interactions that go beyond simple contact points, allowing for refined motion estimation in both contact and non-contact scenarios.
% In reality, individuals frequently engage in more complex interactions with their surroundings, such as sitting on a sofa or leaning against a table. Capturing these nuanced interactions requires a more sophisticated understanding of both semantic and geometric environmental details.

Therefore, this study focuses on effectively leveraging human-environment interactions to enhance full-body motion estimation with sparse tracking signals by utilizing both semantic and geometric aspects of environmental information. Semantic information about the environment is applied to refine poses that involve no direct contact with the environment, providing contextual cues that support realistic estimation of non-contact motions. The geometric constraints from the environment prevent collisions between environmental point clouds and the human model, correcting unreasonable poses in cases of direct physical interactions, such as sitting on furniture or touching objects. By integrating joint uncertainty estimation with semantic and geometric environmental constraints, our method reduces ambiguity in sparse observations and enhances the robustness and accuracy of motion estimation. The contributions of this paper are summarized as follows:


% Semantic understanding can enhance pose estimation results even when the body is not in direct contact with the environment. Additionally, geometric constraints regarding human-object contact interact with the geometric information of environmental point clouds and human skinning data, preventing collisions between environmental points and the human model and thus correcting unreasonable motion estimates. The contributions of this paper are summarized as follows:


% Through interactions and contact with the environment, more constraints can be provided for full-body pose estimation, thereby improving the robustness and accuracy of the estimates. However, existing methods often overlook the interaction between the human body and the environment, beyond simple foot-to-ground contact. In real life, people often engage in more complex interactions with their surroundings, such as sitting on a sofa or leaning on a table. This study's core focus is how to effectively utilize human-environment interactions to assist wearable device-based motion reconstruction. The key lies in constraining pose estimation through semantic and geometric aspects of environmental information. Semantic understanding of the environment can improve pose estimation results when the body is not in direct contact with it; while geometric constraints of human and object contact interact through the geometric information of environmental point clouds and human skinning data, preventing environmental points from embedding into the human model and thus correcting unreasonable pose estimates.

% 将一些HMDPoser、SparsePoseer这种加传感器的解决方案，但是由于侵入感不太行。在引到我们这加上环境的解决方案。点出和我们相似的是S2Fusion，但是他们有xxx缺点，我们的insight是什么。总结贡献点如下：
%To address the issue of high uncertainty in joint rotations caused by sparse observations in VR-based motion capture, existing research \cite{ponton2023sparseposer, dai2024hmd, ponton2024dragposer} has attempted to mitigate this by adding additional sensors to the pelvis and legs. 
%These advanced methods achieve accurate and robust motion capture results by incorporating additional measurements. However, such setups are more closely aligned with research on motion reconstruction based on sparse IMUs \cite{huang2018deep, jiang2022transformer, yi2022physical, zhang2024dynamic}. While they tend to yield better reconstruction results, they may negatively impact the user experience. 
%These advanced methods improve accuracy and robustness in motion capture by incorporating additional sensor measurements. However, such setups are more aligned with research on motion reconstruction using sparse IMUs \cite{huang2018deep, jiang2022transformer, yi2022physical, zhang2024dynamic}. Although they often produce better reconstruction results, they may compromise the overall user experience. 

\begin{itemize}
    \item We propose a novel multi-stage learning framework capable of robustly and accurately estimating users' full-body motion from sparse tracking signals, effectively utilizing semantic and geometric constraints derived from the environment.

     \item This framework introduces an uncertainty-aware 3D motion estimation module based on transformers. This approach effectively addresses the ill-posed problem caused by the absence of lower-body observations, which could effectively express the multiple motion hypotheses.

    % \item For environmental information, we consider both the semantic characteristics and geometric structural constraints of the environment on human pose estimation. We introduce a semantic consistency-aware attention module and a COAP loss term that effectively correct pose estimates with high uncertainty in contact and non-contact scenarios.
    \item To refine motion estimation, we integrate both semantic and geometric constraints of the environment. This includes a semantic consistency-aware attention module and a physics-based collision scoring loss term, which together correct pose estimates with high uncertainty in both contact and non-contact scenarios.
    
    \item Extensive quantitative and qualitative experiments demonstrate that our proposed method achieves state-of-the-art performance across three public datasets and excels in scenarios with frequent environmental interactions, significantly outperforming competing methods.
    
    
\end{itemize}
